Large Language Models(LLMs) on Tabular Data: Prediction, Generation, and Understanding -- A Survey

Recent breakthroughs in large language modeling have facilitated rigorous exploration of their application in diverse tasks related to tabular data modeling, such as prediction, tabular data synthesis, question answering, and table understanding. Each task presents unique challenges and opportunities. However, there is currently a lack of comprehensive review that summarizes and compares the key techniques, metrics, datasets, models, and optimization approaches in this research domain. This survey aims to address this gap by consolidating recent progress in these areas, offering a thorough survey and taxonomy of the datasets, metrics, and methodologies utilized. It identifies strengths, limitations, unexplored territories, and gaps in the existing literature, while providing some insights for future research directions in this vital and rapidly evolving field. It also provides relevant code and datasets references. Through this comprehensive review, we hope to provide interested readers with pertinent references and insightful perspectives, empowering them with the necessary tools and knowledge to effectively navigate and address the prevailing challenges in the field.

==> 03_prediction_internal.tex <==
\section{LLMs for predictions}
\label{prediction}


Several studies have leveraged LLMs for prediction in tabular data. This section will delve into the existing methodologies and advancements in two categories of tabular data: standard feature-based tabular data and time series data. Time series prediction differs from normal feature-based tabular data since the predictive power heavily relies on the past. For each category, we divide it into different steps which include preprocessing, fine-tuning, and target augmentation. Preprocessing explains how different prediction methods generate input to the language model. Preprocessing includes serialization, table manipulation, and prompt engineering. Target augmentation maps the textual output from LLMs to a target label for prediction tasks. At the end, we will briefly cover domain-specific prediction methods using LLMs.

\subsection{Dataset}
For task-specific fine-tuning, most datasets used for the prediction task are from UCI ML, OpenML, or a combo of 9 datasets created by ~\citep{manikandan2023language}. Details of the datasets are in Table~\ref{table/prediction_dataset}. OpenML has the highest number of datasets, but the size of the largest dataset is only 5600 rows. Half of the datasets in UCI ML collections are relevant to medical use cases. 
Thus, the combo of 9 datasets is recommended for benchmark \footnote{GitHub repository link \url{https://Github.com/clinicalml/TabLLM/tree/main/datasets}} since it contains larger size datasets and more diverse feature sets. For general fine-tuning,  published methods choose the Kaggle API\footnote{Link to the pre-trained data \url{https://Github.com/Kaggle/kaggle-api}} as it has 169 datasets, and its datasets are very diverse. 


\begin{table}[h]
\centering
\begin{tabular}{lcl}
\hline
\textbf{Dataset} & \textbf{Dataset Number} & \textbf{Papers that used this dataset} \\ \hline
OpenML           & 11                          & \cite{dinh2022lift, manikandan2023language} \\ 
Kaggle API       & 169                         & \cite{hegselmann2023tabllm, wang2023unipredict, zhang2023foundation} \\ 
Combo            & 9                           & \cite{hegselmann2023tabllm, wang2023unipredict, zhang2023foundation} \\ 
UCI ML           & 20                           & \cite{manikandan2023language,slack2023tablet} \\ 
DDX              & 10                           & \cite{slack2023tablet} \\ 
\hline
\end{tabular}
\caption{Combo is the combination of the following dataset in the form of dataset name (number of rows, number of features): Bank (45,211 rows, 16 feats), Blood
(748, 4), California (20,640, 8), Car (1,728, 8), Creditg (1,000, 20), Income (48,842, 14), and Jungle (44,819,
6), Diabetes (768, 8) and Heart
(918, 11).  }
\label{table/prediction_dataset}
\end{table}

\subsection{Tabular prediction}
\input{tabs/prediction}
\textbf{Preprocessing} 
Preprocessing in LLM-based tabular prediction involves steps like table manipulation, serialization, and prompt engineering, which have been discussed earlier. Specifically, some LLM-based prediction methods incorporated a statistical summary of the tabular data as part of the input to LLM. Serialization in the prediction task is mostly Text-based (refer to Section ~\ref{trends:serialization}).  Prompt engineering includes incorporating task-specific cues and relevant samples into the prompt (refer to Section ~\ref{trends:serialization}). The various preprocessing methods are illustrated in Table~\ref{table:target seralization} and discussed in detail below.



% Some methods create serialization through handcrafting or domain experts. 
As one of the earliest endeavors, LIFT~\citep{dinh2022lift} tried a few different serialization methods, such as feature and value as a natural sentence such as "The column name is Value"  or a bunch of equations, such as $col_{1} = val_{1}, col_{2} = val_{2}, ...$. The former achieves higher prediction accuracy, especially in low-dimensional tasks. The same conclusion was drawn in TabLLM~\citep{hegselmann2023tabllm} where they evaluated 9 different serialization methods along with a description for the classification problem. They found that a textual enumeration of all features: 'The column name is Value', performs the best. For medical prediction, they mimic the thinking process of medical professionals as prompt engineering and found that LLM makes use of column name and their relationships in few-shot learning settings.

In a subsequent study, TABLET~\citep{slack2023tablet} included naturally occurring instructions along with examples for serialization. In this case, where the task is for medical condition prediction, naturally occurring instructions are from consumer-friendly sources, such as government health websites or technical references such as the Merck Manual. It includes instructions, examples, and test data points. They found that these instructions significantly enhance zero-shot F1 performance. However, experiments from TABLET revealed that LLMs tend to ignore instructions, even with examples, leading to prediction failures. Along this fashion, more studies tested a more complex serialization and prompt engineering method rather than a simple concatenation of feature and value for serialization. 

The schema-based prompt engineering usually includes background information about the dataset, a task description, a summary, and example data points. Summary Boosting\citep{manikandan2023language} serializes data and metadata into text prompts for summary generation. This includes categorizing numerical features and using a representative dataset subset selected via weighted stratified sampling based on language embeddings. Serilize-LM~\citep{jaitly2023better} introduces 3 novel serialization techniques that boost LLM performance in domain-specific datasets. They included related features in one sentence to make the prompt more descriptive and easier to understand for LLM. Take car classification as an example, attributes like make, color, and body type are now combined into a single richer sentence. It leverages covariance to identify the most relevant features and either label them critically or add a sentence to explain the most important features. Finally, they converted tabular data into LaTeX code format. This LaTeX representation of the table was then used as the input for fine-tuning our LLM by just passing a row representation preceded by \texttt{hline} tag without any headers. 

Another work worth mentioning is UniPredict~\citep{wang2023unipredict}, which reformats metadata by consolidating arbitrary input M to a description of the target and the semantic descriptions of features. Feature serialization follows a "column name is value" format. The objective is to minimize the difference between the output sequence generated by the adapted LLM function and the reference output sequence generated from target augmentation (represented by serialized target). To make LLMs applicable to multiple tabular datasets at the same time, Generative Tabular Learning (GTL) was proposed by~\cite{zhang2023foundation}.  It includes two parts: 1) the first part specifies the task background and description with optionally some examples as in-context examples(Prompt Engineering); 2) the second part describes feature meanings and values of the current instance to be inferred(Serialization); LIFT and TabLLM have been benchmarked by at least 3 other papers. The code for both methods is available. \footnote{Here is the Github repo for TABLET \url{https://Github.com/dylan-slack/Tablet}, TabLLM \url{https://Github.com/clinicalml/TabLLM} and LIFT \url{https://Github.com/UW-Madison-Lee-Lab/LanguageInterfacedFineTuning}}  

Some other methods leverage an LLM to rewrite the serialization or perform prompt engineering.  TabLLM~\citep{hegselmann2023tabllm} showed that LLM is not good for serialization because it is not faithful and may hallucinate.  Summary Boosting\citep{manikandan2023language}  uses GPT3 to convert metadata to data description and generate a summary for a subset of datasets in each sample round. TABLET~\citep{slack2023tablet} fits a simple model such as a one-layer rule set model or prototype with the 10 most important features on the task’s full training data. It then serializes the logic into text using a template and revises the templates using GPT3. Based on their experiments, it was found that contrary to the naturally occurring instructions, LLM-generated instructions do not significantly improve performance. 


\textbf{Target Augmentation} LLMs can solve complex tasks through text generation, however, the output is not always controllable~\citep{dinh2022lift}. 
As a result, mapping the textual output from LLMs to a target label for prediction tasks is essential. This is called target augmentation~\citep{wang2023unipredict}. A straightforward but labor-intensive way is manual labeling, as was used by Serilize-LM~\citep{jaitly2023better}. To be more automatic, LIFT~\citep{dinh2022lift} utilizes $\#\#\#$ and $@@@$ to demarcate question-answer pairs and signify the end of generation. These markers prompt the LLM to position answers between $\#\#\#$ and $@@@$. This approach significantly aligns most generated answers with the intended labels. Additionally, to address potential inaccuracies in inference outputs, LIFT conducts five inference attempts, defaulting to the training set's average value if all attempts fail. In streamlining the two-step approach, TabLLM~\citep{hegselmann2023tabllm} incorporates the use of Verbalizer~\citep{cui2022prototypical} to map the answer to a valid class. To calculate AUCROC or AUCPR, the probability of the output is necessary. Thus, Verbalizer proves advantageous for closed-source models by enabling the assignment of output probability. UniPredict~\citep{wang2023unipredict} has the most complicated target augmentation. They transform the target label into a set of probabilities for each class via a function called “augment”. Formally, for a target $T$ in an arbitrary dataset $D$, they define a function $augment(T) = {(C, P)}$, where $C$ are new categories of targets with semantic meaning and P are the assigned probabilities to each category. They extend the target into categorical one-hot encoding and then use an external predictor to create the calibrated probability distributions. This replaces the 0/1 one-hot encoding while maintaining the final prediction outcome. Formally, given the target classes $t \in {0, ..., |C|}$ and target probabilities $p \in P$, they define a function serialize target(t, p) that serializes target classes and probabilities into a sequence formatted as “class ${t_{1}} : {p_{1}}$, ${t_{2}} : {p_{2}}$, . . . ”. We give an example for each method in~\ref{table:target_augmentation}


\textbf{Inference Only Prediction} Some work uses LLMs directly for prediction without fine-tuning, we refer to these approaches as inference-only prediction. TABLET~\citep{slack2023tablet} utilizes models like Tk-Instruct~\citep{wang2022supernaturalinstructions} 11b, Flan-T5~\citep{chung2022scaling} 11b, GPT-J~\citep{black2022gptneox20b} 6b, and ChatGPT to inference the model, but finds out that a KNN approach with feature weights from XGBoost surpasses Flan-T5 11b in performance using similar examples and instructions. Summary Boosting~\citep{manikandan2023language} creates multiple inputs through the serialization step. The AdaBoost algorithm then creates an ensemble of summary-based weak learners. While non-fine-tuned LLMs struggle with continuous attributes, summary boosting is effective with smaller datasets. Furthermore, its performance is enhanced using GPT-generated descriptions by leveraging existing model knowledge, underscoring the potential of LLMs in new domains with limited data. However, it does not perform well when there are many continuous variables. For any new LLM-based prediction method without any fine-tuning, we suggest benchmarking LIFT and TABLET. LIFT is the first LLM-based method for inference-only prediction. TABLET shows significantly better performance than LIFT with 3 different base models. 

\textbf{Fine-tuning} 
 For studies involving fine-tuning, they typically employ one of two distinct approaches.
 The first involves training an LLM model on large datasets to learn fundamental features before adapting it to specific prediction tasks. The second takes a pre-trained LLM and further trains it on a smaller, specific prediction dataset to specialize its knowledge and improve its performance on the prediction. LIFT~\citep{dinh2022lift} fine-tunes pre-trained language models like GPT-3 and GPT-J using Low-Rank Adaptation (LoRA) on the training set. They found that LLM with general pretraining could improve performance. However, the performance of this method does not surpass the in-context learning result.  TabLLM~\citep{hegselmann2023tabllm} uses T0 model~\citep{sanh2021multitask} and T-few~\citep{liu2022few} for fine-tuning. TabLLM has demonstrated remarkable few-shot learning capabilities, outperforming traditional deep-learning methods and gradient-boosted trees. TabLLM’s efficacy is highlighted by its ability to leverage the extensive knowledge encoded in pre-trained LLMs from these models, requiring minimal labeled data. However, the sample efficiency of TabLLM is highly task-dependent. Other research also leverages T0 as based model. \citet{jaitly2023better} uses T0~\citep{sanh2021multitask}. Compared to TabLLM, it is trained using Intrinsic Attention-based Prompt Tuning (IA3)~\citep{liu2022few}. However, this method only works for a few short learning, worse than baseline when the number of shots is more or equal to 128. T0 model~\citep{sanh2021multitask} is commonly used as the base model for tabular prediction fine-tuning. 

UniPredict~\citep{wang2023unipredict} trains a single LLM (GPT2) on an aggregation of 169 tabular datasets with diverse targets and observes advantages over existing methods. This model does not require fine-tuning LLM on specific datasets. Model accuracy and ranking are better than XGBoost when the number of samples is small. The model with target augmentation performs noticeably better than the model without augmentation. It does not perform well when there are too many columns or fewer representative features. GTL~\citep{zhang2023foundation}  fine-tunes LLaMA to predict the next token. They leverage 115 tabular datasets. To balance the number of instances across different datasets, they randomly sample up to 2,048 instances from each tabular dataset for GTL. They employed GTL which significantly improves LLaMA in most zero-shot scenarios. Based on the current evidence, we believe that fine-tuning on large number of datasets could further improve the performance. However, both UniPredict and GTL have not released their code yet.

\textbf{Metric} Among all tabular prediction methods surveyed, AUC is mostly commonly used metric for classification prediction and RMSE is mostly commonly used metric for regression~\ref{tab:prediction} 

\begin{table}[h]
\centering
\begin{tabular}{p{5cm}p{4cm}p{7cm}}
\hline
\textbf{Methodology} & \textbf{Method} & \textbf{Example} \\ \hline
Feature name + Feature Value + Predicted Feature Name  & \cite{dinh2022lift, hegselmann2023tabllm} & Car Brand is Land Rover. Year is 2017. Repair claim is \\ 
Task Background + Feature meaning + Feature Value + Predicted Feature meaning& \cite{zhang2023foundation} & The task is about fraud repair claim prediction. The brand of car is Land Rover. The produce year is 2017. The repair claim of the car is \\
Dataset Summary + LLM Processed Feature + Task & \cite{manikandan2023language} & Larger car is always more expensive. This is a 2017 Land Rover. Therefore, this car repair claim is (Fraudulent or Not Fraudulent): \\ 
Latex Format of features value + Task & \cite{jaitly2023better} & Is this car repair claim fraudulent? Yes or No? \\ 
Expert Task Understanding + Label + Task & \cite{slack2023tablet} & Identify if the car repair claim is fraudulent. An older car is more likely to have a fraudulent repair claim. Features Car Brand: Land Rover Year: 2017. Answer with one of the following: Yes | No \\ 
Dataset description + Feature meaning + Feature Value + Task & \cite{wang2023unipredict} & The dataset is about fraud repair claims. Car Brand is the brand of car. The year is the age when the car is produced. The features are: Car Brand is Land Rover. The year is 2017. Predict if this car repair claim is fraudulent by Yes for fraudulent, No for not fraudulent \\ \hline
\end{tabular}
\caption{Method and Example for different preprocessing for general predictive tasks. The example is to predict if a car repair claim is fraudulent or not.} 
% \qnote{the example column has some issues}}
\label{table:target seralization}
\end{table}


% \label{prediction:no_finetuning}
% TABLET~\citep{slack2023tablet} leverages naturally occurring instructions for result interpretation or fitting a prototypes and rulesets classifier. It utilizes models like Tk-Instruct~\citep{wang2022supernaturalinstructions} 11b, Flan-T5~\citep{chung2022scaling} 11b, GPT-J~\citep{black2022gptneox20b} 6b, and ChatGPT. In-context instructions significantly enhance zero-shot F1 performance. However, biases in LLMs against correctly classifying certain instances are noted, and often, LLMs ignore instructions, leading to prediction failures. Contrastingly, a KNN approach with feature weights from XGBoost surpasses Flan-T5 11b in performance using similar examples and instructions. 
% Summary Boosting\citep{manikandan2023language} explores LLMs as weak learners in a boosting framework for tabular data, serializing data and metadata into text prompts for summary generation. This includes categorizing numerical features and using a representative dataset subset selected via weighted stratified sampling based on language embeddings. The AdaBoost algorithm then creates an ensemble of summary-based weak learners. While non-finetuned LLMs struggle with continuous attributes, summary boosting is effective with smaller datasets, with GPT-generated descriptions enhancing performance by leveraging existing model knowledge, underscoring the potential of LLMs in new domains with limited data. However, it does not perform well when there are many continuous variables. 

%LIFT~\citep{dinh2022lift} converts dataset into sentences by format it as a list of strings or a list of equations. It then fine-tuning pretrained language model(GPT3, GPTJ) with LORA on the obtained sentences.  It uses ### for question and answer separation It uses @@@ for end of generation. It put answers in between. To avoid invalid inference, it inference for 5 times and return the average value of the training set if all attempts fail. It shows contextual information of columns improve accuracy. LIFT performs well in low dimensional tasks. LIFT can be used of rdata generation. In Context Learning is comparable with finetuning. LIFT could benefit from language model pretraining. TABLET: It leverages naturally occurring instructions such as technical professional reference or title instructions for the result. Alternativly, it fits a one layer decision tree or presenting the probability of target classes equal to given the value of 10 most important features. It leverages Tk-Instruct 11b and Flan-T5 11b , GPT-J 6b, ChatGPT. Incontext instructions increase zero-shot F1 performance for Flan-T5 11b by 44 percent on average and 13 percent for ChatGPT on TABLET. LLMs are highly-biased against classifying certain instances correctly. It seems that LLMS often ignore instriuctions and fail to predict specific instances correctly even with examples. Through flipped instructions. It does not follow instructions provided in-context. KNN with feature weights from XGBoost is better than Flan T5 11b using the same examples and naturally occurring instructions.  Zero shot learner: explores the use of Large Language Models (LLMs) as weak learners in a boosting framework, particularly for tabular data. In this approach, tabular data and metadata are serialized into text prompts, enabling LLMs to generate summaries. This process includes binning numerical features into categories like “low,” “medium,” and “high.” The study uses a representative subset of the dataset for efficiency, selected via weighted stratified sampling based on language embeddings. After that, the AdaBoost algorithm is employed to create an ensemble of these summary-based weak learners. A key observation is that LLMs, without finetuning, struggle with continuous attributes. However, the approach, termed Summary Boosting, is notably effective with smaller datasets. The research highlights that GPT-generated descriptions enhance performance, leveraging the model's existing knowledge for predictions. This study underlines the potential of LLMs in new domains, especially where data quantity is limited.


% \subsection{Finetuning}

% LIFT, as described by \citep{dinh2022lift}, transforms datasets into sentences by formatting them as lists of strings or equations and fine-tunes pretrained language models like GPT-3 and GPT-J using LORA on these sentences. It employs $###$ and $@@@$ for question-answer separation and end of generation, respectively, placing answers in between. To mitigate invalid inferences, LIFT conducts five inference attempts, defaulting to the training set's average value if all fail. Contextual information from columns is shown to enhance accuracy, especially in low-dimensional tasks, making LIFT suitable for data generation and showing that In Context Learning is comparable to fine-tuning. Moreover, pretraining language models could further benefit LIFT. However, the performance of this method does not surpass in context learning result. 

% TabLLM~\citep{hegselmann2023tabllm} evaluates 9 different serialization methods and find that a textual enumeration of all features 'The column name is Value' perform the best. For medical data, it mimics medical professional for serialization. It uses T0 model~\citep{sanh2021multitask} and t few~\citep{liu2022few-shot} for finetuning. It uses verbalizer~\citep{cui2022prototypical} to map the answer to a valid class. TabLLM outperforms traditional deep-learning methods and gradient-boosted trees, in few-shot learning scenarios. TabLLM’s efficacy is highlighted by its ability to leverage the extensive knowledge encoded in pre-trained LLMs, requiring minimal labeled data. It found out that LLM actually make use for feature name and their relationships in few shot settings. However, The sample efficiency of TabLLM is highly task-dependent.  Based on this paper, LLM is not good for serialization because it is not faithful and may hallucinate. 

% \citep{jaitly2023better} introduces 3 novel serialization technicals which boosts LLM performance in domain specific datasets. It combines few feature into one sentence to make it natural. For car classification as a example, attributes like make, color and body type are now combined into a single richer sentence. It leverage covariance to identify most relevant features and either label them critical or adding a sentence to explain what are most important feature. Finally, it converts tabular data into LaTeX code format. This LaTeX representation of the table was then used as the input for fine-tuning our LLM by just passing a row representation preceded by hline tag without any headers. It adopt a manual specification for this mapping. It uses  T0~\citep{sanh2021multitask}. It is trained using Intrinsic Attention-based Prompt Tuning (IA3)~\citep{liu2022few}. However, this method only works for few short learning, worse than baseline when number of shots more or equal to 128.  

% UniPredict~\citep{wang2023unipredict} trains a sngle LLM on an aggregation of 169 tabular datasets with diverse targets and observe advantage over existed methods. This model does not require to finetune LLM on specific datasets. For serialization, it refromats meta data. It consolidates arbitrary input M to a description of the target to predict and the semantic descriptions of features. Feature serialization is using the format column is value, .... The objective is to minimize the difference between the output sequence generated by the adapted LLM function and the reference output sequence generated from target augmentation (represented by serialize target). For output, they transform the target label into a set of probabilities for each class via a function called “augment”. Formally, for target T in an arbitrary dataset D, they define a function $augment(T) = {C, P}$, where C are new categories of targets with semantic meaning and P are the assigned probabilities to each category. They extend the target into categorical one-hot encoding and then use an external predictor to create the calibrated probability distributions. This replaces the 0/1 one-hot encoding while maintaining the final prediction outcome. Formally, given the target classes $t \in {0, ..., |C|}$ and target probabilities $p \in P$, they define a function serialize target(t, p) that serializes target classes and probabilities into a sequence formatted as “class ${t_{1}} : {p_{1}}$, ${t_{2}} : {p_{2}}$, . . . ”. Model accuracy and ranking is better than XGBoost when the number of samples is small. The model with target augmentation performs noticeably better than the model without augmentation. It does not perform well when there are two many columns or less representative features. 
  


\subsection{Time Series Forecasting }

% \qnote{we can keep this section.. just need to add a claim saying time series datasets do not fully follow the "order invariant" properties }

Compared to prediction on feature-based tabular data with numerical and categorical features, time series prediction pays more attention to numerical features and temporal relations. Thus, serialization and target augmentation are more relevant to how to best represent numerical features. Many papers have claimed that they use LLM for time series. However, most of these papers use LLM which is smaller than 1B. We will not discuss these methods here. Please refer to ~\citep{jin2023lm4ts} for a complete introduction of these methods.  

\textbf{Preprocessing} PromptCast~\citep{xue2022prompt} uses input time series data as it is and converts it to a test format with minimal description of the task and converts the target as a sentence to be the output. ZeroTS~\citep{gruver2023large} claims that the number is not encoded well in the original LLM encoding method. Thus, it encodes numbers by breaking them down by a few digits or by each single digit for GPT-3 and LLaMA, respectively. It uses spaces and commas for separation and omitting decimal points. Time LLM~\citep{jin2023time} involves patching time series into embeddings and integrating them with word embeddings to create a comprehensive input. This input is complemented by dataset context, task instructions, and input statistics as a prefix. TEST~\citep{sun2023test} introduces an embedding layer tailored for LLMs, using exponentially dilated causal convolution networks for time series processing. The embedding is generated through contrastive learning with unique positive pairs and aligning text and time series tokens using similarity measures. Serialization involves two QA templates, treating multivariate time series as univariate series for sequential template filling. 

\textbf{Target Augmentation} In terms of output mapping, ZeroTS~\citep{gruver2023large} involves drawing multiple samples and using statistical methods or quantiles for point estimates or ranges. For Time-LLM~\citep{jin2023time},  the output processing is done through flattening and linear projection.  The target augmentation method of ZeroTS is easy to implement~\footnote{The code is in \url{https://Github.com/ngruver/llmtime}}. 

\textbf{Inference Only Prediction} Similar to feature-based tabular prediction, researchers explored LLMs' performance for time series forecasting without fine-tuning. ZeroTS~\citep{gruver2023large} examines the use of LLMs like GPT-3~\citep{brown2020language} and LLaMA-70B~\cite{touvron2023llama} directly for time series forecasting.  It evaluates models using mean absolute error (MAE), Scale MAE, and continuous ranked probability score (CRPS), noting LLMs' preference for simple rule-based completions and their tendency towards repetition and capturing trends. The study notes LLMs' ability to capture time series data distributions and handle missing data without special treatment. However, this approach is constrained by window size and arithmetic ability, preventing it from further improvement. 

\textbf{Fine-tuning} Fine-tuning the model for time series prediction is more commonly seen in current research. PromptCast~\citep{xue2022prompt} tried the method of inference-only prediction or fine-tuning on task-specific datasets. It shows that larger models always perform better. Time LLM~\citep{jin2023time} presents a novel approach to time series forecasting by fine-tuning LLMs like LLaMa~\cite{touvron2023llama} and GPT-2~\citep{brown2020language}.  Time-LLM is evaluated using metrics symmetric mean absolute percentage error (SMAPE), mean absolute scaled error (MSAE), and overall weighted average (OWA). It demonstrates notable performance in few-shot learning scenarios, where only 5 percent or 10 percent of the data are used. This innovative technique underscores the versatility of LLMs in handling complex forecasting tasks.  For TEST~\citep{sun2023test}, soft prompts are used for fine-tuning. The paper evaluates models like Bert, GPT-2~\citep{brown2020language}, ChatGLM~\citep{zeng2023glm130b}, and LLaMa~\cite{touvron2023llama}, using metrics like classification accuracy and RMSE. However, the result shows that this method is not as efficient and accurate as training a small task-oriented model. In general, currently, LLaMa is used as the base model by most papers we surveyed. 

\textbf{Metric} MAE is the most common metric. Continuous Ranked Probability Score (CRPS) as it captures distributional qualities, allowing for comparison of models that generate samples without likelihoods. CRPS is considered an improvement over MAE as it does not ignore the structures in data like correlations between time steps.  Symmetric Mean Absolute Percentage Error (SMAPE) measures the accuracy based on percentage errors, Mean Absolute Scaled Error (MASE) is a scale-independent error metric normalized by the in-sample mean absolute error of a naive benchmark model, and Overall Weighted Average (OWA) is a combined metric that averages the ranks of SMAPE and MASE to compare the performance of different methods. Among those metrics, MAE and RMSE are mostly used and benchmarked by at least half of our surveyed methods in time series. 



\begin{table}[h]
\centering
\begin{tabular}{p{4cm}p{4cm}p{7cm}}
\hline
\textbf{Method} & \textbf{Used Paper} & \textbf{Example} \\ \hline
Adding Special Token before and after the answer & \cite{dinh2022lift} & \verb|### {Category} @@@| \\ 
Verbalizer & \cite{hegselmann2023tabllm} & \verb|Output -> {category1: probability1, .}| \\ 
Specific Prefix & \cite{manikandan2023language, slack2023tablet} & Please answer with category 1, category 2, ... \\ 
Predict probability and recalibrate & \cite{wang2023unipredict} & \verb|{category1: probability1}| => Calibrated by XGBoost \\ \hline
\end{tabular}
\caption{Target Augmentation method, used papers and examples}
\label{table:target_augmentation}
\end{table}

 
% \citep{gruver2023large} examines the use of LLMs like GPT-3~\citep{brown2020language} and LLaMA-70B~\cite{touvron2023llama} for time series forecasting. They claim that the number is not encoded well in original LLM encoding method. Thus, it encodes numbers differently, breaking them down by a few digits for GPT-3 or by each digit for LLaMA. It uses spaces and commas for separation and omitting decimal points. For outputs, the method involves drawing multiple samples and using statistical methods or quantiles for point estimates or ranges. The study notes LLMs' ability to capture good distributions and handle missing data without special treatment. It evaluates models using MAE, Scale MAE, and CRPS, noting LLMs' preference for simple rule-based completions and their tendency towards repetition and capturing trends. However, the limited window size and arithmetic ability limit this approach's potential for further improvement. 
% Time LLM~\citep{jin2023time} presents a novel approach to time series forecasting by finetuning LLMs like LLaMa~\cite{touvron2023llama} and GPT-2~\citep{brown2020language}. The method involves patching time series into embeddings and integrating them with word embeddings to create a comprehensive input. This input is complemented by dataset context, task instructions, and input statistics as a prefix. The output is done through flatten and linear projection.  Time-LLM is evaluated using metrics like SMAPE, MSAE, and OWA. It demonstrates notable performance in few-shot learning scenarios, where only 5 percent or 10 percent of the data are used. This innovative technique underscores the versatility of LLMs in handling complex forecasting tasks. 
% TEST~\citep{sun2023test} focuses on adapting LLMs for time series tasks. It introduces an embedding layer tailored for LLMs, using exponentially dilated causal convolution networks for time series processing. The embedding is generated through contrastive learning with unique positive pairs and aligning text and time series tokens using similarity measures. Serialization involves two QA templates, treating multivariate time series as univariate series for sequential template filling. Soft prompts are used for fine-tuning. The paper evaluates models like Bert, GPT-2~\citep{brown2020language}, ChatGLM~\citep{zeng2023glm130b}, and LLaMa~\cite{touvron2023llama}, using metrics like Classification Accuracy and RMSE. However, the result shows that this method is not efficient and accurate as training a small task oriented model.





\subsection{Application of Prediction using LLM}
\textbf{Medical Prediction} 
Medical data such as electronic health records (EHR) have clinical events with timestamps. The BERT-based model could capture the long-term dependencies among events such as diabetes. Thus, LM based models~\citep{mcmaster2023adapting,steinberg2021language, rasmy2021med, li2020behrt} perform better than XGBoost. 
However, these models only focused on predicting a small fraction of the International Statistical Classification of Diseases and Related Health Problems (ICD) codes. Currently, Meditab~\citep{wang2023meditab} aims to create a foundation model in the medical field.
% Meditab~\citep{wang2023meditab} uses GPT-3.5~\citep{brown2020language} to transform tabular data into text, focusing on key values. It then applies linearization, prompting, and sanity checks to ensure accuracy and reduce errors. It then trains a multi-task learning model on domain specific data, generate pseudo labels for supplementary datasets, and refine these using data Shapley scores for quality. It then pretrains the model on the refined dataset and fine-tune with original data. The final model supports both zero-shot and few-shot learning for new datasets. It uses GPT3.5~\citep{brown2020language} via OpenAI’s API for the data consolidation and enhancement. It uses UnifiedQA-v2-T5~\citep{khashabi2022unifiedqa} for the sanity check. It uses pretrained BioBert~\citep{Lee_2019} as classifier. An extensive evaluation of MediTab’s performance in supervised learning, few-shot learning, and zero-shot prediction in medical domain. 
For preprocessing, Meditab utilizes GPT-3.5 \cite{brown2020language} to convert tabular data into textual format, with a focus on extracting key values. Subsequently, it employs techniques such as linearization, prompting, and sanity checks to ensure accuracy and mitigate errors. For fine-tuning, the system further leverages multitask learning on domain-specific datasets, generates pseudo-labels for additional data, and refines them using data Shapley scores. Pretraining on the refined dataset is followed by fine-tuning using the original data. The resulting model supports both zero-shot and few-shot learning for new datasets. GPT-3.5 accessed via OpenAI’s API facilitates data consolidation and augmentation, while UnifiedQA-v2-T5 \cite{khashabi2022unifiedqa} is employed for sanity checks. Additionally, Meditab utilizes a pre-trained BioBert classifier \cite{Lee_2019}. The system undergoes thorough evaluation across supervised, few-shot, and zero-shot learning scenarios within the medical domain, demonstrating superior performance compared to gradient-boosting methods and existing LLM-based approaches. However, it may have limited applicability beyond the medical domain.\footnote{ The code is available at \url{https://Github.com/RyanWangZf/MediTab}.} for tabular prediction tasks specifically in the medical domain. Like other methods, they also use a precision-recall curve (PRAUC) for evaluation. PRAUC is useful in imbalanced datasets, which is always the case for medical data. 

% TreeDistill~\citep{yang2023effective} was build upon the notion that some emergent abilities of LLMs can be transferred to smaller models through distillation. The authors tries to create a small description of science table. It use synthetic data from LLMs, using GPT 3.5 Turbo~\citep{brown2020language} to generate two reasoning and description through CoT. It uses another LLM to verify generated answer and summary. It finetunes a small model given task and reasoning to get summary. It uses T5-~\citep{raffel2023exploring}base and T5-large and BART as baselines~\citep{lewis2019bart}, However, it only evaluates on one dataset(SciGen~\citep{moosavi2021scigen}) with CoT data as input to smaller model. However, the smaller model does not perform as well as GPT3.5.  

% TreeDistill~\citep{yang2023effective} is founded on the idea that certain emergent capabilities of LLMs can be transferred to smaller models through distillation. The authors aimed to create concise descriptions of scientific tables. They utilized synthetic data from LLMs, employing GPT 3.5 Turbo~\citep{brown2020language} to generate two sets of reasoning and descriptions via CoT. Another LLM was employed to validate the generated answers and summaries. Subsequently, a small model was fine-tuned based on the task and reasoning to produce a summary. Baselines such as T5-base, T5-large, and BART~\citep{lewis2019bart} were utilized. However, the evaluation was conducted solely on the SciGen dataset~\citep{moosavi2021scigen} with CoT data as input for the smaller model. Unfortunately, the smaller model did not perform as effectively as GPT3.5.

\textbf{Financial Prediction}  FinPT~\citep{yin2023finpt} presents an LLM-based approach to financial risk prediction. The method involves filling tabular financial data into a pre-defined template, prompting LLMs like ChatGPT and GPT-4 to generate natural-language customer profiles. These profiles are then used to fine-tune large foundation models such as BERT~\citep{devlin-etal-2019-bert}, employing the models' official tokenizers. The process enhances the ability of these models to predict financial risks, with Flan-T5 emerging as the most effective backbone model in this context, particularly across eight datasets. For financial data, FinBench contains 10 datasets with varied training set sizes (from 2k - 140k) and feature sizes (from 9 - 120)
~\footnote{The dataset is in \url{https://huggingface.co/datasets/yuweiyin/FinBench} and the code for FinPT is in \url{https://Github.com/YuweiYin/FinPT}}.

\textbf{Recommendation Prediction} CTRL~\citep{li2023ctrl} proposes a novel method for Click Through Rate (CTR) prediction by converting tabular data into text using human-designed prompts, making it understandable for language models. The model treats tabular data and generated textual data as separate modalities, feeding them into a collaborative CTR model and a pre-trained language model such as ChatGLM~\citep{zeng2023glm130b}, respectively. CTRL employs a two-stage training process: the first stage involves cross-modal con trastive learning for fine-grained knowledge alignment, while the second stage focuses on fine-tuning a lightweight collaborative model for downstream tasks. The approach outperforms all the SOTA baselines including semantic and collaborative models over three datasets by a significant margin, showing superior prediction capabilities and proving the effectiveness of the paradigm of combining collaborative and semantic signals. However, the code for this method is not available. They use LogLoss and AUC to evaluate the method. For LogLoss, A lower bound of 0 for Logloss indicates that the two distributions are perfectly matched, and a smaller value indicates a better performance.




% \subsection{Use LLM as prior for prediction model}
% LLM Prior: Categorical columns are augmented by using aChatGPT to rank categories, which are then mapped to integers and standardized.
% The ChatGPT uses column headers of continuous variables to predict if the column is positively or negatively correlated with the target attribute and a soft prior is applied to the classifier model. Prior is applied to MonotonicLR through regularizing beta the average effective gradient over all categories for each column. Since MonotonicLR is based on LR it is easy to analyze and interpretate. Every baseline is evaluated on datasets with 1) raw data, 2) ordered categorical columns 3) one-hot encoded categorical columns. The performance is not as good as TabPFN. It requires manual checking for each feature to understand positivity which makes it harder to do in reality. Not seems an efficient way to use LLM 

% VectorLLM: Analytical tasks on tables tackle, in general, estimation of statistical properties of the records. Conditional estimate of one row over all others. OpenAI’s ada-002 and BAAI’s BGE-large-en-v1.5 improve performance.  vectorize  text and high-cardinality features are vectorized using a language model before feeding into a classification algorithm. They find Language model can extract valuable knowledge from text features. It achieves better performance but does not really compare with state of the arts in the domain.  

% TabText: focuses on creating embeddings from tabular data. The method involves formatting the data into text sentences and combining tables into paragraphs. These paragraphs are embedded using Longformer, a variant of BERT, and then used for predictions with tree-type models. The approach requires less preprocessing, especially benefiting hard-to-classify examples, and acts as data enrichment in the embedding space. 


 




